Efficient Differentiable Simulation of Articulated Bodies

We present a method for efficient differentiable simulation of articulated bodies. This enables integration of articulated body dynamics into deep learning frameworks, and gradient-based optimization of neural networks that operate on articulated bodies. We derive the gradients of the forward dynamics using spatial algebra and the adjoint method. Our approach is an order of magnitude faster than autodiff tools. By only saving the initial states throughout the simulation process, our method reduces memory requirements by two orders of magnitude. We demonstrate the utility of efficient differentiable dynamics for articulated bodies in a variety of applications. We show that reinforcement learning with articulated systems can be accelerated using gradients provided by our method. In applications to control and inverse problems, gradient-based optimization enabled by our work accelerates convergence by more than an order of magnitude.

==> shortcuts.tex <==
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath,amssymb,amsthm}

\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother

\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% \usepackage{algpseudocode}

\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries


\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}

\newcommand\timess{\mathbin{\!\times\!}}

\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

\newcommand\yourname[1]{\textcolor{blue}{Name says: #1}}

\newcommand\ylq[1]{\textcolor{black}{#1}}

\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

\def\rot#1{\rotatebox{90}{#1}}

\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}


% \newcommand\PD[2]{\frac{\partial #1}{\partial #2}}
\newcommand\adj[2]{\overline{ #1}_{#2}}

==> tex/method_backup.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/arti.pdf}
    \vspace{-4mm}
    \caption{The workflow of a simulation step. Assume there are $n_q=6$ DoF, the input state is an $n_q\times 3$ matrix containing the position, velocity, and control input of each joint. The forward dynamics will traverse the articulated body sequentially three times. This process is hard to parallelize and will generate a large number of intermediate results. After the forward dynamics is a collision resolving step with collision detection and an iterative Gauss-Seidel solver. The size of initial states is much smaller than intermediate results but it has all the information to resume all the variables. }
    \label{fig:arti}
\vspace{-3mm}
\end{figure*}



\section{Preliminaries}
\mypara{Articulated Body Dynamics}.
For the forward simulation, we choose the recursive O(n) method, Articulated Body Algorithm (ABA)~\cite{Featherstone2007RigidBD,Coumans2015bullet,Coumans2020tiny}, which is widely used in mainstream articulated body simulators ~\cite{todorov2012mujoco,Coumans2015bullet,lee2018dart}. In each simulation step $k$, the states $\xx^k$ of the system consist of generalized coordinates and their velocities $\xx^k = [\qq^{k},\Dot{\qq}^{k}]\in \mathbb{R}^{2 n_q\times 1}$, where $n_q$ is the degrees of freedom of this system. Assume that each joint can be actuated by a torque, then there is an $n_q$-dimension control signal $\uu^k\in \mathbb{R}^{n_q\times 1}$. the discretized dynamics at this step can be written as $\ff^{k+1}(\uu^k,\xx^{k},\xx^{k+1})=0$.

\mypara{Adjoint Method}.
The adjoint method has been used to compute gradients in a variety of tasks~\cite{mcnamara2004fluid,Holl2020,david2020radiative,chen2018neural}. In our pipeline, we can concatenate the variables in the entire time sequence and get $\xx=[\xx^{1},\xx^{2},...,\xx^{n_t}]\in \mathbb{R}^{n_t \cdot 2n_q\times 1}$ and control input $\uu=[\uu^{1},\uu^{2},...,\uu^{n_t}]\in \mathbb{R}^{n_t \cdot n_u\times 1}$, where $n_t$ is the number of simulation steps. The concatenated dynamics equation can similarly write as $\ff=[\ff^1,\ff^2,...,\ff^{n_t}]=0$. When there is an learning or optimization problems, we would usually define a scalar objective function $\Phi(\xx,\uu)$. To get the derivative of this function w.r.t. control input $\uu$, one needs to compute,
\begin{equation}
    \frac{d\Phi}{d\uu}=\PD{\Phi}{\uu}+\PD{\Phi}{\xx}\frac{d\xx}{d\uu}.
    \label{eq:diff_u}
\end{equation}
$\PD{\Phi}{\uu}$ is easy to compute for each single simulation step. But it is prohibitively expensive to directly solve $\PD{\Phi}{\xx}\frac{d\xx}{d\uu}$ because $\frac{d\xx}{d\uu}$ will be a $2n_qn_t\times n_qn_t$ matrix. 

Instead, we differentiate the dynamics $\ff(\xx,\uu)=0$ and obtain the constraint $\PD{\ff}{\xx}\frac{d\xx}{d\uu}=-\PD{\ff}{\uu}$. Apply adjoint method~\cite{mcnamara2004fluid}, and $\PD{\Phi}{\xx}\frac{d\xx}{d\uu}$ equals to,
\begin{equation}
  -\RR\trans\PD{\ff}{\uu} \textrm{ \hspace{5mm} such that \hspace{5mm} } (\PD{\ff}{\xx})\trans\RR=(\PD{\Phi}{\xx})\trans
  \label{eq:adj_back}
\end{equation}
Since the dynamics equation for one step only involves few previous steps, the sparsity of $\PD{\ff}{\uu}$ and $\PD{\ff}{\xx}$ makes it easier to solve Equation~\ref{eq:adj_back}.

$\PD{\Phi}{\uu}-\RR\trans\PD{\ff}{\uu}$ is called the adjoint of $\uu$, which is equivalent to the gradients by our substitution. In the following derivation, we denote the adjoint (gradient) of a variable $\sss$ as $\overline{\sss}$.

% In fact, we will show in Section~\ref{sec:adj} that the way we calculate $\RR^k$ equals to computing the gradients of $\xx^k$.


\section{Efficient Differentiation in Time and Space}
In this section, we introduce the algorithm for the gradient computation in articulated simulation. For faster differentiation, the gradients of articulated body dynamics are computed by the adjoint method. We derive the adjoint of time integration, collision resolving, and forward dynamics in a reverse order. Since we can now mange the computation and storage manually, checkpoint method is introduced into our pipeline to further save the memory usage. The detailed scheme for checkpointing is finalized by analysis on the workload of the simulation as shown in Figure~\ref{fig:arti}.

% In general, we adopt the classical three-pass iterative method~\cite{Featherstone2007RigidBD} for the forward simulation, as shown in Figure~\ref{fig:arti}.
% In order to balance between memory and time consumption, we save the simulation states at each time step as checkpoint, and resume the one-step simulation when backpropagating the gradients. Inside each step, we use the adjoint method to compute the gradients in the reverse order of the simulation flow.
% \begin{algorithm}[h]
% \caption{Forward articulated simulation}
% \label{alg:simulation}
% \begin{algorithmic}[1]
% %   \State $\xx^0 \gets \bZero$
%   \State $\xx^1 \gets$ initial condition 
%   \For{$t=1$ {\bfseries to} $n-1$}
%     \State $\uu^t \gets$ control input
%     \State save\_checkpoints$(\xx^{t},\uu^{t})$
%     \State $\xx_d \gets$ forward\_dynamics$(\xx^{t},\uu^{t})$
%     \State $\xx_c \gets$ collision\_resolving$(\xx_d)$
%     \State $\xx^{t+1} \gets$ time\_integration$(\xx_c)$
%     % \State $\II^t, \pp^t \gets$ update\_kinematics($\xx^k$)
%     % {\color{red}TODO}
%   \EndFor
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[h]
% \caption{Backward articulated simulation}
% \label{alg:simulation}
% \begin{algorithmic}[1]
%   \State $\xx^{1,...,n_t},\uu^{1,...,n_t} \gets$ checkpoints
%   \State $\Phi(\xx,\uu) \gets$ objective function
%   \State $\RR^{n_t}=\PD{\Phi}{\xx^{n_t}}$
%   \For{$t=n_t-1$ {\bfseries to} $1$}
%     \State $\xx^t,\uu^t \gets$ reload checkpoints
%     \State $\xx_d, \xx_c\gets$ forward\_simulation$(\xx^{t},\uu^{t})$
%     % \State $ \gets$ adj_time\_integration$(\xx_d,\xx_c)$
%     % \State $ \gets$ adj_collision\_resolving$(\xx_d)$
%     \State $ \gets$ collision\_resolving$(\xx_d)$
%     \State $\xx^{t} \gets$ time\_integration$(\xx_c)$
%     \State $\II^t, \pp^t \gets$ update\_kinematics($\xx^k$)
%     {\color{red}TODO}
%   \EndFor
% \end{algorithmic}
% \end{algorithm}


\subsection{Adjoint Method on Articulated Simulation}
\label{sec:adj}
As shown in Figure~\ref{fig:arti}, the one-step articulated simulation can be split into 3 modules, in a sequential order.
During backward differentiation, as illustrated in Figure~\ref{fig:fb}, we will follow the blue arrows first to reload the checkpoints and resume the simulation. Then, we will compute the gradients in the reverse order (along with red arrows) using the adjoint method. 


\mypara{Time integration.}
The backpropagation starts from the time integration. As an example, for a simulation sequence with $n_t=3$ steps and an integrator with two temporal horizon, the constraints $(\PD{\ff}{\xx})\trans\RR=(\PD{\Phi}{\xx})\trans$ in Equation~\ref{eq:adj_back} can be expanded as,
\begin{equation}
\left[
\begin{array}{ccc}
(\PD{\ff^1}{\xx^1})\trans & (\PD{\ff^2}{\xx^1})\trans & 0  \\
0 & (\PD{\ff^2}{\xx^2})\trans & (\PD{\ff^3}{\xx^2})\trans  \\
0 & 0 & (\PD{\ff^3}{\xx^3})\trans
\end{array}\right]
\left[
\begin{array}{c}
\RR^1\\
\RR^2\\
\RR^3
\end{array}\right]=
\left[
\begin{array}{c}
(\PD{\Phi}{\xx^1})\trans\\
(\PD{\Phi}{\xx^2})\trans\\
(\PD{\Phi}{\xx^3})\trans
\end{array}\right]
\end{equation}\label{eq:adj_constraints}
If using explicit Euler integrator, we have $\PD{\ff^k}{\xx^k}=\II$. To begin with, $\RR^{n_t}=\PD{\Phi}{\xx^{n_t}}$. And the following $\RR^k$ can be computed iteratively by, 
\begin{equation}
    \RR^k=(\PD{\Phi}{\xx^k})\trans-(\PD{\ff^{k+1}}{\xx^k})\trans\RR^{k+1}, k=1,2,..,n_t-1.
\end{equation}
\label{eq:adj_r}
When $\RR^k$ backpropagates through time, the gradients $\overline{\uu^k}$ can also be computed by Equation~\ref{eq:adj_back}. In fact, by the way we calculate $\RR^k$, it equals to the gradients of $\xx^k$. Other parameters can also be computed in a similar way as $\overline{\uu^k}$.  

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/forward_backward.pdf}
    \vspace{-4mm}
    \caption{Differentiate articulated body dynamics by checkpoints and adjoint methods. The diagram on the top is the forward simulation at step $k$. Our simulator will store the states $\qq^k, \Dot{\qq}^k$ and control input $\uu^k$. During backpropagation, as illustrated in the bottom, the checkpoints will be reloaded, with which the simulator run one forward step again and resume the intermediate variables. Beginning with the gradients from $k+1$ step, we will use adjoint method to sequentially compute the gradients of each variables through time integration, constraint solver, and forward dynamics.}
    \label{fig:fb}
\vspace{-3mm}
\end{figure}
\mypara{Collision resolving.} 
The collision resolving step consists of collision detection and a collision solver. Upon receiving the gradients $\overline{\xx}$ from time integrator, the collision solver need to pass the gradients to detection, and then to the forward dynamics. 
In our collision solver, we follow the pipeline in \cite{Jakub2013} and construct a Mixed Linear Complementarity Problem (MLCP), 
\begin{equation}
\begin{split}
    &\aa = \AA\xx+\bb\  \\
    \textrm{ s.t. \hspace{2mm} } \bm{0}\leq &\aa \perp \xx\geq \bm{0}\textrm{\hspace{1mm} and \hspace{1mm}} \cc_- \leq \xx  \leq\cc_+ 
\end{split}
\label{eq:mlcp}
\end{equation}
where $\xx$ is the new collision-free state, $\AA$ is the inertial matrix, $\bb$ contains the relative velocities, and $\cc_-, \cc_+$ are the lower bound and upper bound constraints, respectively. We use projected Gauss-Seidel (PGS) method to solve this MLCP. This iterative solve trades off accuracy for speed such that the constraints $\aa\trans\xx=0$ might not hold on termination. In this more general case where the solution is not guaranteed to satisfy constraints, the implicit differentiation for solvers~\cite{Belbute2018,Qiao2020Scalable,Liang2019} no longer works. Instead, we design a reverse version of the PGS solver using adjoint method to compute the gradients. More details of the solver is in the Appendix. Basically, it mirrors the PGS, substituting the original operators with their adjoints.   
This step passes the gradients from the collision-free states to the forward dynamics.

\mypara{Forward dynamics.}
Our articulated body simulator updates its forward dynamics in a chain-like fashion as shown in Figure~\ref{fig:arti} the green blocks. Each operation in the forward simulation has its corresponding adjoint operation in the backward pass. To compute those gradients, we derive a bunch of adjoint rules for operators in Spatial Algebra~\cite{Featherstone2020spatial} and linear algebra.

% To illustrate, the acceleration of the $i$-th DoF, $\Ddot{q}_i\in\mathbb{R}$, is computed by
% \begin{equation}
%     \Ddot{q}_i = D_i^{-1}(u_i-\UU_i^T\aa_i),
% \end{equation}
% where $D_i, u_i\in\mathbb{R}$ are scalars and $\UU, \aa\mathbb{\RR}^6$ are spatial vectors. Once we get the gradient $\overline{\Ddot{q}}_i$, we can propagate it to its inputs $\Dot{D}_i=-(u_i-\UU_i^T\aa_i)$

% a spatial vector $\pp_i=[\ww,\vv]\in\mathbb{R}^6$ representing the bias force of the $i$-th link is the sum of an external force $[\ff_1, \ff_2]\in\mathbb{R}^6$ and a cross product of two temporal variables $[\ww_1,\vv_1], [\ww_2,\vv_2]\in\mathbb{R}^6$,
% \begin{equation}
% \left[
% \begin{array}{c}
% \ww\\
% \vv
% \end{array}\right]=
% \left[
% \begin{array}{c}
% \ww_1 \times \ww_2+\vv_1\times\vv_2\\
% \ww_1\times\vv_2
% \end{array}\right]
% \end{equation}\label{eq:sm-crossf}

As a simple example, a spatial vector $\pp_i=[\ww,\vv]\in\mathbb{R}^6$ representing the bias force of the $i$-th link is the sum of an external force $[\ff_1, \ff_2]\in\mathbb{R}^6$ and a cross product of two temporal variables $[\ww_1,\vv_1], [\ww_2,\vv_2]\in\mathbb{R}^6$,
\begin{equation}
\left[
\begin{array}{c}
\ww\\
\vv
\end{array}\right]=
\left[
\begin{array}{c}
\ff_1+\ww_1 \times \ww_2+\vv_1\times\vv_2\\
\ff_2+\ww_1\times\vv_2
\end{array}\right]
\end{equation}\label{eq:sm-crossf}
Once we get the gradient $[\overline{\ww}, \overline{\vv}]$ of $\pp_i=[\ww,\vv]$, we can propagate it to its inputs,
\begin{equation}
\begin{split}
\left[
\begin{array}{c}
\adj{\ww}{1}\\
\adj{\vv}{1}
\end{array}\right]&=
\left[
\begin{array}{c}
-\adj{\ww}\times\ww_2-\adj{\vv}\times\vv_2 \\
-\adj{\ww}\times\vv_2
\end{array}\right] \\
\left[
\begin{array}{c}
\adj{\ww}{2}\\
\adj{\vv}{2}
\end{array}\right]&=
\left[
\begin{array}{c}
\adj{\ww}\times\ww_1\\
\adj{\ww}\times\vv_1+\adj{\vv}\times\ww_1
\end{array}\right]
,
\left[
\begin{array}{c}
\adj{\ff}{1}\\
\adj{\ff}{2}
\end{array}\right]=
\left[
\begin{array}{c}
\overline{\ww}\\
\overline{\vv}
\end{array}\right] \\
\end{split}
\end{equation}\label{eq:adjdemo}

This example shows the adjoint of one forward operation. The time and space complexity of the original operation and its adjoint are the same as the forward simulation. More details about the adjoint operations can be found in the Appendix.


\subsection{Memory Effective Checkpointing}
The algorithm we use in the forward articulated simulation is shown in Figure.~\ref{fig:arti}. In each simulation step, there are 5 sequential modules:
(a) perform the forward kinematics from the root link to the leaf links; (b) update the forces from the leaves to the root; (c) update the accelerations from the root to the leaves; (d) detect and resolve collisions; and (e) perform time integration. Although the input and output variables have relatively small DoFs (positions, velocities, and accelerations), there are a lot more intermediate values computed during the process.

Although this is fine with normal simulation because the temporary space for intermediate results can be reused for each step, it is not the case for differentiable simulation because the entire computation graph needs to be stored. This will cause memory consumption to explode when the simulation horizon goes up.

The need for scaling to larger simulation steps motivates our checkpointing method for saving memory.
Instead of saving the entire computation graph, we choose to store only the states of each step.
This is optimal because (a) the states of each step have the smallest size among all essential information in order to replicate the simulation step, (b) finer checkpoints are not useful because at least one step of intermediate results is needed to be stored in order to do the simulation. (c) sparser checkpoints will use less memory to store but it requires to resume multiple steps, costing more memory for resuming making differentiation of time integration difficult.
Figure~\ref{fig:fb} demonstrates the process of checkpointing. During the forward simulation, we store the states of the simulation before the steps begin. During the backpropagation, we load the stored values back and redo the forward (one-step) simulation again to generate the computation graph, and compute the gradients accordingly.

In summary, assuming the simulation step consists of two parts below:
\begin{equation}
    \ZZ^k=G(\xx^{k-1}),\xx^k=F(\ZZ^k)
\label{equ:intermediate}
\end{equation}
where $\ZZ^k$ represents all the intermediate results in between.
After each step, we free the space storing $\ZZ^k$ immediately to save the space, only storing $\xx^k$.
During the backpropagation, we re-compute  $\ZZ^k$ from $\xx^{k-1}$ again using Equation~\ref{equ:intermediate}.
After that, we can use the adjoint method in the next subsection to compute the gradients of the previous step:
\begin{gather}
    \overline{\ZZ^k}=backwardF(\ZZ^k, \xx^k, \overline{\xx^k})\\
    \overline{\xx_{k-1}}=backwardG(\xx_{k-1},\ZZ_k,\overline{\ZZ^k})
\end{gather}
where $\overline{*}$ is the adjoint of the variable.

% \mypara{Update Kinematics.}
% In this module, we compute the articulated momentum and inertia matrix for each joint in a top-down manner, based on the current state $\qq$. We show one example of computing the world-space position below:
% \begin{gather}
%     \xx_k=\OO_p\dd_{k-p}+\xx_p
% \end{gather}
% where $\xx_k$ is the position of the k-th joint, with $p$ being its parent joint, $\OO$ the joint orientation, and $\dd_{k-p}$ the local displacement.
% Here the transformation matrix is linear to the input variable, $\xx_p$ and $\dd_{k-p}$ (we skip the complicated one , $\OO_p$, the details of which are listed in the Appendix), so the adjoint is straightforward:
% \begin{gather}
%     \RR_{\xx_p}=\sum_k \RR_{\xx_k}\\
%     \RR_{\dd_{k-p}}=\OO_p\trans\RR_{\xx_k}
% \end{gather}
% Note however that, the order of the computation of adjoints is reversed, i.e. bottom-up in this module instead of top-down.

% \mypara{{\color{red}TODO}}

% \subsection{Forward and backward of Articulated Body Dynamics}
%\mypara{Storing variables} during the forward simulation for later use in backward differentiation is necessary for differentiable physics. 
%One principle is that enough information needs to be stored during the forward pass, or we cannot efficiently resume the intermediate variables and compute the gradients. On the other hand, storing the entire computation history, like most of the auto-diff tools did, might not be the optimal choice because it will take up extra memory and time. To better understand the workload of articulated body simulation and analyze how to differentiate it, we plot a diagram of one simulation step in Figure~\ref{fig:arti}.

%In the pipeline, a simulation loop in each step consists of three stages: forward dynamics, collision resolving, and time integration. At the forward dynamics stage, the algorithm will traverse the links for three iterations to, \romannumeral1. perform the forward kinematics from the root link to the leaf links; \romannumeral2. update the forces from the leaves to the root; \romannumeral3. update the accelerations from the root to the leaves. Note that the initial state vector $\xx^k=[\qq^{k},\Dot{\qq}^{k},\uu^k]\in\mathbb{R}^{n_q\times 3}$ only has 3 dimensions for each DoF, but the size of intermediate variables (spatial velocities, forces, inertia matrices, and etc.) associate with each DoF can be 100 times more than the initial size. In this sense, the state vector can be viewed as a bottleneck of the simulation, that it is a vector containing all the information for the simulation step but of the minimal size. Based on this observation, we only store the state vectors $\xx^k$ during forward simulation. Instead of simply storing the entire computational graph, our strategy effectively reduces the vast majority of memory usage. Typically, the dimension of $\xx^k$ is less than 100, which means the memory used for storage is around 1KB per step. A long 
%simulation sequence with $1\times 10^6$ steps only occupied 1 GB memory, within the durable size for a modern computer.

%In Section~\ref{sec:autodiff} we will show that our method can save more than 99\% of the peak memory when compared with auto-diff tools. Less memory usage enables longer simulation length, so that users can simulate large scenes and more complex motion. With more simulation steps, we can also set smaller time step for better accuracy and stability of the simulation.
 
%\mypara{Deriving the gradients} is another key point when we choose to manually manage the memory and differentiate the physics.
%Unlike fluid or deformable solid where individual grids and particles are rather independent, links in an articulated body are organized in a fix order. The data flow in Figure~\ref{fig:arti} cannot be accelerated by parallelization, and there is no explicit governing equation for the derivative of state vectors $\xx^k:=[\qq^{k\trans},\Dot{\qq}^{k\trans},\uu^k]\in \mathbb{R}^{n_q\times 3}$. Instead, the gradients need to be computed iteratively in a more fine-grained level.

%% \subsection{Adjoints of Articulated Body Dynamics}
%% In equation~\ref{eq:adj_r}, the most challenging parts in each simulation step are $\PD{\ff^{k+1}}{\xx^k}$ and $\PD{\ff^k}{\uu^k}$. Since those two terms only depends on the current step, the computational history before or after the step $k$ is irrelevant. Therefore, the differentiation in each step only involve with its own checkpoint and can be conducted independently. 
%Figure~\ref{fig:fb} is an illustration of the backpropagation using adjoint method. During each forward simulation, the positions $\qq^k$, velocities $\Dot{\qq}^k$, and torques $\uu^k$ will be stored as checkpoints. When applying the adjoint method in backward, we will first reload the checkpoints and run the simulation again, which will resume the intermediate results in forward dynamics, constraint solver, and the time integration stages. Then, the gradients of all the variables can be computed in a reverse order. 

%The adjoints of time integration is similar to the example in Equation~\ref{eq:adj_constraints}. For the collision resolving, we use the iterative projected Gauss-Seidel method to solve the Mixed Linear Complementary Problem (MLCP), which trades off accuracy for speed. In this more general case where the solution is not guaranteed to satisfy constraints, the implicit differentiation for solvers~\cite{Belbute2018,Qiao2020Scalable,Liang2019} no longer works. To compute the gradients, we instead design a reverse version of the solver using adjoint method. After that, we compute the adjoints of collision detection and pass the gradients to forward dynamics.

%To differentiate the three stages in forward dynamics, we derive the adjoint rules for operators in Spatial Algebra~\cite{Featherstone2020spatial} and linear algebra. The details of the adjoint method for the solver and forward dynamics can found in the Appendix. 

%%In short, we derive the adjoint rules for the Spatial Algebra~\cite{Featherstone2020spatial}, and the Gauss-Seidel solver for Mixed Linear Complementary Problem (MLCP).


